Uncertainty separation via ensemble quantile regression

This paper introduces a novel and scalable framework for uncertainty estimation and separation with applications in data driven modeling in science and engineering tasks where reliable uncertainty quantification is critical. Leveraging an ensemble of quantile regression (E-QR) models, our approach enhances aleatoric uncertainty estimation while preserving the quality of epistemic uncertainty, surpassing competing methods, such as Deep Ensembles (DE) and Monte Carlo (MC) dropout. To address challenges in separating uncertainty types, we propose an algorithm that iteratively improves separation through progressive sampling in regions of high uncertainty. Our framework is scalable to large datasets and demonstrates superior performance on synthetic benchmarks, offering a robust tool for uncertainty quantification in data-driven applications.

==> sections_old/Evaluation.tex <==
\section{Evaluation}
\subsection{Toy}
\label{sec:toy}
\begin{figure*}
    \centering        
    \includegraphics[width=0.9\textwidth]{figs/fitting_results.pdf}
    \caption{Uncertainty estimation in Ensembles quantile regression and the resulting epistemic and aleatoric uncertainty.}
    \label{fig:toy_fitting_result}
\end{figure*}
In this work, we aim to fit the function 
\[
y_1 = \sin \left(\sqrt{x_1^2 + x_2^2}\right)
\]
\[
y_2 = x \cdot \cos\left(\sqrt{x_1^2 + x_2^2}\right) \cdot \cos(x_2)
\]
using both Deep Ensembles (DE) and Ensemble Quantile Regression (E-QR). To make the problem more challenging and realistic, we introduce two specific regions in the input space that lack representative data, as well as two regions that exhibit irreducible aleatoric noise modeled as 
\[
\mathcal{N}(0, 0.3).
\]

\subsubsection{Ensembles of Quantile Regression (E-QR)}
Figure \ref{fig:toy_fitting_result} illustrates the aleatoric and epistemic uncertainty calculated by the E-QR model for both outputs. Notably, aleatoric uncertainty appears to leak into the epistemic uncertainty plot. \navid{Consider testing whether epistemic uncertainty can leak into aleatoric uncertainty, either in this experiment or another setup.}

Using Algorithm \ref{alg:u_separation}, we can generate an uncertainty map. By iteratively focusing on uncertain regions and selectively filling them with additional data, the true aleatoric uncertainty regions can be accurately recovered.


\subsubsection{Deep Ensembles (DE)}
\begin{figure*}
    \centering        
    \includegraphics[width=0.9\textwidth]{figs/fitting_result_DE.pdf}
    \caption{Uncertainty estimation in Deep Ensembles and the resulting epistemic and aleatoric uncertainty.}
    \label{fig:toy_DE_fitting_result}
\end{figure*}

In Deep Ensembles, acquiring a reliable estimate of aleatoric uncertainty is significantly more challenging, which complicates the separation of uncertainties. Consequently, Algorithm \ref{alg:u_separation} requires more iterations to achieve an acceptable level of separation. Figure \ref{fig:toy_DE_fitting_result} illustrates the uncertainty separation at iteration 0 and the progressive improvement in separation as Algorithm \ref{alg:u_separation} is executed over 7 iterations.

\navid{Can epistemic leak into aleatoric? run experiment}
\navid{show that naive sampling require much more samples to yield the same results }



==> sections_old/Intro.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, uncertainty estimation has become an essential aspect of machine learning, especially for applications that demand high reliability in decision-making, such as autonomous driving \cite{kendall2017uncertainties}, and medical diagnosis \cite{lambrou2010reliable, yang2009using}. Accurate uncertainty estimation not only supports better model interpretability but also helps identify areas where models are likely to make errors, ensuring safety in high-stakes environments.
%

Uncertainty in machine learning is typically categorized into two types: aleatoric uncertainty, which originates from inherent noise or variability in the data, and epistemic uncertainty, which stems from limitations in the model’s knowledge and can potentially be reduced with additional data \cite{hullermeier2021aleatoric}. Separating these two types of uncertainty is essential in applications like Bayesian optimization \cite{ansari2023large}, inverse design \cite{ansari2022autoinverse}, and active learning \cite{ren2021survey}, where understanding the nature of uncertainty influences strategic decisions. 
%
%For instance, in active learning, distinguishing between data-driven and knowledge-based uncertainty helps guide sampling, enabling efficient exploration of the input space.
%
For instance, in Bayesian optimization and inverse design, focusing on epistemic uncertainty directs computational resources toward regions where additional data could improve model performance.

While various methods exist for modeling uncertainty, most approaches cannot effectively scale with increasing dataset size \navid{explain and ref how other BNNs scale worse \cite{ansari2023large}}. Among the techniques capable of handling large-scale data are Deep Ensembles (DE) \cite{Lakshminarayanan2017} and Monte Carlo (MC) dropout \cite{Gal2016}, which can provide uncertainty estimates and some degree of uncertainty separation. However, both methods face limitations across all three key aspects of uncertainty estimation quality:

\begin{itemize}
    \item \textbf{Localization of Uncertainty:} The first and simplest task in uncertainty estimation is identifying regions within the input space that may lead to unreliable predictions, regardless of the type of uncertainty. Effective localization aids in detecting areas where model predictions might lack robustness.

    \item \textbf{Separation of Uncertainties:} The next level involves distinguishing between aleatoric and epistemic uncertainty across the input domain. This distinction is particularly valuable in applications such as Bayesian optimization and active learning, where it is beneficial to avoid exploring regions dominated by irreducible aleatoric noise.

    \item \textbf{Accurate Magnitude Estimation of Uncertainty:} At the highest level of uncertainty estimation, models should not only localize and separate uncertainty but also provide precise magnitude estimates for uncertainty in each prediction.
\end{itemize}



==> sections_old/Method.tex <==
\section{Methodology}
In Section \ref{sec:E_QR}, we describe the ensembling of quantile regression models as an alternative to DE and MC dropout. Then, in Section \ref{sec:separation}, we discuss the shortcomings of scalable Bayesian Neural Networks (BNNs) in uncertainty separation and demonstrate how Algorithm \ref{alg:u_separation} can be used to achieve robust uncertainty separation. In Section \ref{sec:conformal_EC}, we outline how ensemble QR models can be improved using calibration data and conformal scores. Finally, We apply the classic conformal method to further adjust the magnitude of the predicted uncertainty, enhancing the reliability of our estimates.

\subsection{Ensemble Quantile Regression} \label{sec:E_QR}

Quantile regression is a technique used to predict specific quantiles of the target distribution, providing not only a central prediction but also upper and lower bounds, which are essential for uncertainty estimation. Unlike standard regression methods that minimize mean squared error, quantile regression minimizes the \textit{pinball loss} (or quantile loss), which is defined for a quantile level \( q \) as follows:

\begin{equation}
    L_q(y, \hat{y}) = 
    \begin{cases} 
      q \cdot (y - \hat{y}) & \text{if } y \geq \hat{y}, \\
      (1 - q) \cdot (\hat{y} - y) & \text{if } y < \hat{y},
    \end{cases}
\end{equation}

where \( y \) is the true value and \( \hat{y} \) is the predicted quantile. This loss penalizes over- and under-estimations differently based on the quantile \( q \), allowing for asymmetric error handling. For instance, setting \( q = 0.5 \) corresponds to the median prediction \( q_{0.5} \), while \( q = 0.1 \) and \( q = 0.9 \) represent the lower and upper bounds of the distribution, respectively.

After training N instances of QR \navid{appendix implementation}, the ensemble provides a set of predictions for each quantile level. The epistemic uncertainty, which arises from model uncertainty, is estimated using the variance across the ensemble members' predictions for the median quantile \( q_{0.5}(x) \). Specifically, the epistemic uncertainty \( \sigma_\text{epistemic} \) is calculated as:
\[
\sigma_\text{epistemic}(x) = \sqrt{\frac{1}{N} \sum_{i=1}^{N} \left( q_{0.5}^{(i)}(x) - \overline{q_{0.5}}(x) \right)^2 },
\]
where \( q_{0.5}^{(i)}(x) \) is the prediction of the \( i \)-th network for the median quantile, and \( \overline{q_{0.5}}(x) \) is the mean of these predictions:
\[
\overline{q_{0.5}}(x) = \frac{1}{N} \sum_{i=1}^{N} q_{0.5}^{(i)}(x).
\]

The aleatoric uncertainty, is derived from the difference between the upper and lower quantiles predicted by the ensemble \cite{Pearce2018} when $alpha \approx 0.3085$ (\navid{see appendix Section \ref{q_vs_sigma}}). The total uncertainty \( \sigma_\text{total} \) is given by:
\[
\sigma_\text{total}(x) = \frac{1}{N} \sum_{i=1}^{N} \left( q_{1-\alpha}^{(i)}(x) - q_{\alpha}^{(i)}(x) \right).
\]

\navid{explain that instead of fixing alpha to this number we can add a coefficient and use other alphas as well.}

We argue that the separation at this step is not reliable (\navid{section xxx}) so Unlike \cite{Lakshminarayanan2017} we do not combine the uncertainties at this stage.


\subsection{Comparison of DE, MC dropout and QR}

With regards to epistemic uncertainty, Deep Ensembles (DE) and Ensemble Quantile Regression (E-QR) are more powerful than MC dropout. This is because DE and E-QR train several independent models with varying parameters and activation functions, while MC dropout relies on stochastic variations of a single model \navid{\cite{xxx}}.

While the epistemic uncertainty calculation for DE and E-QR is similar, they differ in their mechanisms for predicting aleatoric uncertainty at the level of their sub-networks. DE uses sub-networks trained to directly learn aleatoric uncertainty via the Negative Log Likelihood (NLL) loss, reporting it as a separate output neuron alongside the primary predictions. On the other hand, E-QR subnetworks predict quantiles using the pinball loss, providing an indirect but effective way to estimate aleatoric uncertainty.

Training E-QR is simpler and more stable compared to DE due to the following reasons:
\begin{itemize}
    \item Training with pinball loss is inherently simpler and more stable than NLL loss \navid{why}.
    \item In practice, DE training typically requires two steps: first, optimizing the primary prediction (\(\mu\)) and then using the NLL loss to train the uncertainty (\(\sigma\)) heads (\navid{ref}). This process doubles the computational effort compared to E-QR, where the quantile predictions are learned simultaneously in a single step.
\end{itemize}

Apart from the simplicity of training, we demonstrate in Section \navid{\ref{navid_xxx}} that the quality of aleatoric uncertainty predictions made by E-QR is superior to those of DE. This superiority arises \navid{why?}

\subsection{Uncertainty separation and its challenges}
\label{sec:challenges}

\textbf{Leakage of Aleatoric Uncertainty into Epistemic Uncertainty}

Although epistemic uncertainty is intended to capture only uncertainty due to limited knowledge, in practice, it may inadvertently include aleatoric uncertainty when data is insufficient. This occurs because each subnetwork in an ensemble model is trained on a subsample of the data. If these subsamples are too small, subnetworks may overfit to their specific data rather than generalizing between data points, as expected with an L2 loss function. As a result, aleatoric uncertainty can "leak" into the epistemic uncertainty estimates. This phenomenon is common in both Deep Ensembles and Ensemble Quantile Regression methods. \navid{add an inset figure}

\textbf{Leakage of epistemic uncertainty in aleatoric uncertainty.}


All models studied here rely on fitting mechanisms to model aleatoric uncertainty. DE uses the Negative Log Likelihood (NLL) loss, while E-QR employs the pinball loss to fit upper and lower quantiles. As a result, the accuracy of these predictions depends heavily on the availability of high-quality and sufficient data.
%
In regions with high epistemic uncertainty—due to sparse or insufficient input space coverage—aleatoric uncertainty estimates can become unreliable. This issue is exacerbated by the use of bagging in sub-networks, where only a subsample of data is visible to models attempting to learn aleatoric uncertainty.

\navid{add an inset figure}

Knowing that the root cause of both problems is the lack of data, we propose a progressive sampling strategy in the next section. This strategy focuses on regions where uncertainty is detected, but the type of uncertainty (aleatoric or epistemic) remains unclear. By progressively acquiring additional data in these regions, the model can refine its predictions and better separate the two types of uncertainty.

\subsection{Reliable separation of epistemic and aleatoric uncertainty}
\label{sec:separation}
To reliably separate aleatoric and epistemic uncertainties, we first identify regions where uncertainty is suspected and create a comprehensive uncertainty map by normalizing and combining all available uncertainty maps. In cases with multiple outputs, we focus on the common regions across each output's uncertainty map, as these shared uncertainties are more likely to originate from the data rather than local misfitings specific to individual outputs.

Once this common uncertainty map is established, we gather additional data in the uncertain regions and retrain the models. Iteratively repeating this process diminishes regions of epistemic uncertainty while areas of aleatoric uncertainty remain unchanged. By performing a logical XOR operation between the final uncertainty map and the initial one, we can isolate the initial epistemic uncertainty present in our initial dataset.
% 
Algorithm \ref{alg:u_separation} presents the complete procedure. 




%%%%%%%%%%%%%%%%%%%%%%%%%% Algorithm %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]
\scriptsize % Adjust the font size
\textbf{Input}

$(X, Y)^0$  \hspace{0.4cm}  \textcolor{comment_color}{\tcp{Initial data set}}\
$Q$  \hspace{0.4cm} \textcolor{comment_color}{\tcp{Number of iterations of the main algorithm}}\
$O$  \hspace{0.4cm} \textcolor{comment_color}{\tcp{Number of outputs}}\
$\Phi$  \hspace{0.4cm} \textcolor{comment_color}{\tcp{ Native Forward Process, e.g., a simulation}}\
$T$  \hspace{0.4cm} \textcolor{comment_color}{\tcp{Threshold value for Binarizing the uncertainty map}}\
\textbf{Output}

$U_{E}$, $D_{UE}$ , $P_{UE}$ \hspace{0.4cm} \textcolor{comment_color}{\tcp{Position and value of the separated \textbf{epistemic} regions.}}\
$U_{A}$, $D_{UA}$ , $P_{UA}$ \hspace{0.4cm} \textcolor{comment_color}{\tcp{Position and value of the separated \textbf{aleatoric} regions.}}\

%
\Begin{
    $data set \gets (\mathbf{X^{0}}$,\: $\mathbf{Y^{0}})$\
    
    $f_{BNN}^{0} \xLeftarrow[\text{}]{\text{train}} dataset$ \textcolor{comment_color}{\tcp{Train the BNN surrogate.}}

    $U_A, U_E \gets f_{BNN}^{0}$ \textcolor{comment_color}{\tcp{calculate the uncertainties from the surrogate.}}

     $\min{U_E}, \max{U_E}, \min{U_A}, \max{U_A} \gets \text{\textit{MIN-MAX}}(U_E, U_A)$ 
     \textcolor{comment_color}{\tcp{Extracting the min-max of the uncertainties to be used for scaling.}}
    \For{$i\gets1$ \KwTo $Q$}{
        \For{$ j \gets1$ \KwTo $O$}{

            $\overline{U_E}, \overline{U_A} \gets \textit{Normalizer}(\min{U_E}, \max{U_E}, \min{U_A}, \max{U_A})$ 
              \textcolor{comment_color}{\tcp{Scaling and normalizing both total uncertainty and epistemic uncertainty calculated from the original dataset.}}
            $ \overline{U_{total}^j} = \overline{U_E} + \overline{U_A}$ 
              \textcolor{comment_color}{\tcp{ Adding both normalized uncertainties to make sure all the uncertain regions are captured.}}
            $ \overline{U_{total}^{total}} = \overline{U_{total}^{total}} \times \overline{U_{total}^j}$ 
              \textcolor{comment_color}{\tcp{Multiplying all the total uncertainty maps for all outputs to make sure we only keep the ones that are mutual.}}
            $ (X, Y)^i \gets \textit{Binarize}(\overline{U_{total}^{total}}, T)$
              \textcolor{comment_color}{\tcp{Binarizing the uncertainty map to create a mask for extracting the next batch of data $(X, Y)^i$.}}
              $data set \gets (X,Y)^i$
              \textcolor{comment_color}{\tcp{Append new data to the old.}}\
              $f_{BNN}^{i} \xLeftarrow[\text{}]{\text{train}} data set$  \textcolor{comment_color}{\tcp{Train the BNN surrogate.}}\
              $U_A^i, U_E^i \gets f_{BNN}^{i}$ \textcolor{comment_color}{\tcp{calculate the uncertainties from the surrogate.}}       
         } 
        }
        $U_{A}, D_{UA} , P_{UA} \gets \overline{U_{total}^{total}}$ \textcolor{comment_color}{\tcp{After sufficient number of iterations the total uncertainty map only contains aleatoric uncertainty.}}
        $U_{A}, D_{UA} , P_{UA} \gets  \overline{U_{total}^{total}} \oplus \overline{U_{total}^{0}}$ \textcolor{comment_color}{\tcp{By comparing the final total uncertainty with the initial one we can determine the epistemic uncertain regions of the initial data.}} 
        
\caption{Uncertainty separation.}
\label{alg:u_separation}
 }
\end{algorithm}



==> sections_old/Related.tex <==
\section{Related work}
\label{sec:related}

Uncertainty estimation in machine learning has gained significant attention, particularly in the context of deep learning models. The separation of epistemic and aleatoric uncertainty is essential for reliable decision-making processes in various applications. Deep Ensembles (DE), introduced by \citep{Lakshminarayanan2017}, have been widely adopted due to their effectiveness in providing uncertainty estimates by averaging predictions from multiple neural networks trained independently \cite{Lakshminarayanan2017}. While DE has the potential to estimate both epistemic and aleatoric uncertainty we will show in many cases it fails to do so.

Monte Carlo (MC) dropout is another popular technique for uncertainty estimation, where dropout is applied during both training and inference to approximate Bayesian neural networks \cite{Gal2016}. While MC dropout is effective in some cases, it suffers from high computational costs and can lead to overconfident predictions.

Recent advancements have explored the use of quantile regression for uncertainty estimation, which directly predicts the quantile of the target distribution instead of point estimates. This approach has shown promise in capturing the aleatoric uncertainty \cite{Koenker1978}.
To ensemble all these models, \cite{fakoor2023flexible} proposed an aggregation paradigm focused primarily on enhancing aleatoric uncertainty capture through flexible weighting schemes, though they do not address uncertainty separation for epistemic uncertainty.

In Section \navid{xxx} we show that the by ensembling multiple instances of the quantile regression models we can capture the epistemic uncertainty as well.


Our approach builds on these ideas by introducing a novel ensemble of quantile regression models that outperforms traditional DE and MC dropout techniques in uncertainty predictions, estimation accuracy, and training efficiency. 

In Section \navid{xxx}, we demonstrate that under certain conditions, existing methods can misclassify uncertainty types and provide inaccurate predictions. To address these issues, we introduce an algorithm designed to enhance accuracy and reliability in uncertainty separation. Our key contributions tries to improve uncertainty estimation in all three criteria:

\begin{itemize}
    \item \textbf{Ensemble Quantile Regression}: We propose ensembling quantile regression as a robust alternative to Deep Ensembles (DE) and MC dropout, improving the localization of uncertainty.
    \item \textbf{Enhanced Uncertainty Separation}: We identify limitations in Bayesian Neural Networks (BNNs) and introduce a novel algorithm that, through minimal sampling of the Native Forward Process (NFP), enhances uncertainty separation.
\end{itemize}

